Discrepancy-Sensitive Dynamic Fractional Cascading, Dominated Maxima Searching, and 2-d Nearest Neighbors in Any Minkowski Metric

This paper studies a discrepancy-sensitive approach to dynamic fractional cascading. We provide an efficient data structure for dominated maxima searching in a dynamic set of points in the plane, which in turn leads to an efficient dynamic data structure that can answer queries for nearest neighbors using any Minkowski metric. We provide an efficient data structure for dominated maxima searching in a dynamic set of points in the plane, which in turn leads to an efficient dynamic data structure that can answer queries for nearest neighbors using any Minkowski metric.

==> intro.tex <==
\section{Introduction}
\emph{Discrepancy theory} deals with the degrees to which point sets 
differ from their expected uniformity
(e.g., see Chazelle~\cite{c-gcdm-99,c-dm-02}).
This theory is usually applied globally, for entire sets, but
we are interested in local notions of discrepancy, 
dealing with how sets differ from their expected uniformity in
small intervals.
This interest is motivated from 
\emph{dynamic fractional cascading}~\cite{cg-fc1ds-86,cg-fc2a-86,mn-dfc-90}.

In fractional cascading~\cite{cg-fc1ds-86,cg-fc2a-86},
we are given a bounded-degree\footnote{We note
    that a catalog graph of 
    degree $d>3$ can be transformed into a degree-3 catalog graph by
    replacing high-degree nodes with complete binary trees.}
\emph{catalog graph} $G$,
such that each vertex $v$ of $G$ stores a catalog $C(v)\subset U$,
for a total order $U$.
\ifFull
The catalogs stored at nodes in $G$ are assumed
to be stored sorted
according to the total order $U$ (and we note that this 
  assumption can be relaxed (for
  example, for sets of disjoint line segments), so that we assume that
  the $C(v)$'s contained in any possible search path all belong to a
  common total order. That is, the partial order defined by
  all of the $C(v)$'s has a common linearization.
Intuitively, a catalog graph $G$ is a data structure and the paths in $G$ are
potential traversals in $G$ that might be needed in order to
answer a given query.
\fi
Given a value $x$ belonging to the total order for a
path $P$ in $G$, a query for $x$ in $P$ searches
for $x$ in the catalog $C(v)$ for each vertex $v$ in $P$.
If insertions and deletions are allowed in the $C(v)$'s,
then we have the
``dynamic fractional cascading''~\cite{mn-dfc-90} problem.
Static fractional cascading solutions due to 
Chazelle and Guibas~\cite{cg-fc1ds-86,cg-fc2a-86}
allow for queries to be performed in a
path of length $k$ in time $O(\log n + k)$, where $n$ is the total size of
all the catalogs, and 
dynamic fractional cascading solutions due to Mehlhorn and 
N{\"a}her~\cite{mn-dfc-90}
show that such queries can be done in a dynamic setting
in $O(\log n + k\log\log n)$
time, with updates taking $O(\log n\log\log |U|)$ amortized time.
\ifFull
Thus, achieving a dynamic data fractional cascading data structure
has an increased complexity.
Moreover, this complexity seems inherently difficult to eliminate in the
worst case, as it is based on the use of fairly sophisticated data
structures that seem necessary in order to handle updates to adjacent
catalogs that are very different from one another.
\fi
The reduced efficiency 
of dynamic fractional cascading seems to come from its need to dynamically
handle discrepancy.
Our interest in this paper, therefore, is to address discrepancy
head on---to design a scheme for dynamic fractional cascading 
that is \emph{discrepancy sensitive}.
\ifFull
The motivation for such an approach is that there are a number 
of applications, motivated by real-world scenarios, where the
discrepancies between adjacent catalogs are not that great.
\fi

\ifFull
\subsection{Real-World Nearest Neighbor Queries}
Suppose, for example, 
that in a given region, such as a downtown area or
university campus, there are sensors that keep 
track of different physical entities, such as police
kiosks, doctors' offices, or coffee shops. When the services of one of these
entities are suddenly and urgently needed---e.g., a robbery is in progress,
someone is having a heart attack, or a paper deadline is looming---there
is a need to quickly compute the position of the entity closest to the
location of the sudden emergency event.
The important observation we make for such real-world scenarios
is that service centers, such as these, are
naturally distributed in a fairly uniform way. 
So if we were to
partition our space according to some reasonable data structuring scheme, 
and apply fractional cascading, we should expect
adjacent catalogs to be fairly similar.

This paper therefore deals with the
questions of how to make such notions of similarity precise and 
to design structures that store and dynamically update the positions of the
entities so that the above-mentioned nearest-neighbor queries can be
efficiently processed. 
The data structures we seek should handle arbitrary insertions and
deletions.
This is necessary in order
to model situations where an entity can suddenly become unavailable or
available: for instance, a doctor who is no longer on call or has
returned from caring
for a patient, a police officer who is busy handling a robbery, or
a coffee shop that has run out of espresso.
% Moreover, the transition of an entity
% between ``available'' and ``unavailable'' need not be close in either time
% or space to its previous transition in the other direction.
%
More formally, our motivating application
can be stated as follows: Given a dynamic set $S$
of $n$ points in the plane of real coordinates $x$ and $y$, we seek to
maintain a data structure that is (i) space-efficient
and (ii) supports fast updates (insertions and deletions), as well as fast
exact nearest-neighbor (NN) queries. 
The query points are not necessarily in $S$, but we allow our
structure to run faster when $S$ can be partitioned into subsets with
low relative local discrepancy.
\fi

\emph{Previous Related Work.}
\ifFull
There is a considerable amount of prior related work on discrepancy theory
and fractional cascading data structures. 
\fi
For prior results in discrepancy theory, for example, please
see the excellent book by Chazelle~\cite{c-dm-02}.
Subsequent to the introduction of fractional cascading by
Chazelle and Guibas~\cite{cg-fc1ds-86,cg-fc2a-86} and its dynamic
implementation by Mehlhorn and 
N{\"a}her~\cite{mn-dfc-90}, there have been many specific uses for
this technique, as well as a generalization, due to
Sen~\cite{s-fcr-95}, based on randomized skip lists, and an extension
for I/O efficiency due to Yap and Zhu~\cite{yz-yalfc-01}.

The prior work on nearest neighbor structures is vast; 
for more detailed reviews, see the surveys by
Alt~\cite{a-nn-01} or Clarkson~\cite{nn_survey}.
\ifFull
Indeed, let us focus here on prior work for planar point sets.
\fi
For static data, there are several ways to achieve 
$O(\log n)$ time for nearest-neighbor queries in the plane, including
constructing a planar point location data structure ``on top'' of  a 
Voronoi diagram (e.g., see~\cite{ps-cgi-85}).
For uniformly distributed data, Bentley, Weide, and
Yao~\cite{bwy-oeta-80} give optimal algorithms for static data, and
Bentley~\cite{b-kd-90} gives an optimal algorithm for the semidynamic
(deletion only) case.
\ifFull
We are not familiar with any previous optimal fully dynamic
algorithms for exact nearest-neighbor queries in uniformly distributed data.
\fi
For approximate nearest-neighbor queries, Arya {\it et
al.}~\cite{amnsw-oaann-98} give an optimal static structure, and
Eppstein {\it et al.}~\cite{egs-sqsdd-05} give an optimal 
dynamic structure.
Finally, for general exact nearest-neighbor queries, Chan~\cite{Chan}
gives a dynamic method that achieves polylogarithmic expected times for
updates and queries.
In addition, there has been some work on nearest-neighbors in
non-Euclidean settings for ``reasonably separated'' uniform point sets (e.g.,
see~\cite{bkl-ctnn-06,kl-nn-04,kr-fnn-02}), but this does work does
not apply efficiently to Euclidean metrics on point sets taken from continuous
uniform distributions.

\emph{Our Results.}
In this paper, we introduce 
a study of a discrepancy-sensitive approach to dynamic
fractional cascading.
Unlike the Mehlhorn-N{\"a}her approach, which assumes a worst-case
distribution for the discrepancies between adjacent catalogs, our
approach is sensitive to these differences.
That is, it runs faster through low-discrepancy neighbors and slower
through high-discrepancy neighbors.
We show, for example, that a search for a value $x$ in 
a collection of catalogs, of size at most $n$,
stored in vertices of a path $P$ can be done in time 
$O(\log n + \sum_{(v,w)\in P} \log \delta_{v,w}(x))$, where
$\delta_{v,w}(x)$ is the relative local discrepancy at 
$x$ of the catalogs stored at the nodes $v$ and $w$ in $G$.
Such a discrepancy-sensitive result is useful in a number of real-world
scenarios, as we show that there are several practical distributions
such that the sum of the relative local discrepancies in the catalogs
belonging to a path of length $k$ is $O(k)$ with high probability.
For example,
we use this approach to provide an efficient data structure for
dominated maxima searching in a dynamic set of uniformly distributed
points in the plane.
This, together with the known fact 
that the expected number of maxima points in an uniformly
distributed set $S$ of $n$ points in $\mathbb{R}^{2}$ is $O(\log n)$,
shows that we can
construct a dynamic data structure that can answer
queries for nearest neighbors in $S$ using any Minkowski metric, where 
insertions and deletions run in $O(\log^2 n)$ expected time and 
queries run in $O(\log n)$ expected time, as well. 
These expectations assume a uniform distribution, but
even with real-life (not uniformly distributed) data we experimentally
observe it to hold.


